MedAide: Information Fusion and Anatomy of Medical Intents via LLM-based Agent Collaboration

In healthcare intelligence, the ability to fuse heterogeneous, multi-intent information from diverse clinical sources is fundamental to building reliable decision-making systems. Large Language Model (LLM)-driven information interaction systems currently showing potential promise in the healthcare domain. Nevertheless, they often suffer from information redundancy and coupling when dealing with complex medical intents, leading to severe hallucinations and performance bottlenecks. To this end, we propose MedAide, an LLM-based medical multi-agent collaboration framework designed to enable intent-aware information fusion and coordinated reasoning across specialized healthcare domains. Specifically, we introduce a regularization-guided module that combines syntactic constraints with retrieval augmented generation to decompose complex queries into structured representations, facilitating fine-grained clinical information fusion and intent resolution. Additionally, a dynamic intent prototype matching module is proposed to utilize dynamic prototype representation with a semantic similarity matching mechanism to achieve adaptive recognition and updating of the agent's intent in multi-round healthcare dialogues. Ultimately, we design a rotation agent collaboration mechanism that introduces dynamic role rotation and decision-level information fusion across specialized medical agents. Extensive experiments are conducted on four medical benchmarks with composite intents. Experimental results from automated metrics and expert doctor evaluations show that MedAide outperforms current LLMs and improves their medical proficiency and strategic reasoning.

==> sections/conclusion.tex <==
\section{Conclusion}


==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}
This is used to test the format of the introduction. Test the citation format, single citation:~\cite{dit}~\cite{gpt1}~\cite{repa}~\cite{sit}, multiple consecutive citations:~\cite {dit,repa,gpt1,sit}. Test for abstract. The arrangement of items on the desk was intentional, though the reasons for this particular order were not immediately clear. A list of tasks was written on a notepad, but its relevance to the day's larger goals remained a subject of internal debate. We often consider the passage of time as a constant, yet our perception of it shifts depending on the circumstances, a fact that has little bearing on the objects in this room. The window offers a view of other buildings, each with its own set of windows and its own internal, unobserved activities. A decision was made to use the blue pen instead of the black one. This choice, while minor, set a certain tone for the subsequent notes that were taken. The sound of distant traffic provided a consistent background hum, a neutral soundtrack to the day's proceedings. Each document was placed into a folder, and each folder was given a label. The system was logical and complete, a small pocket of order. The question of what would happen next was present, but not pressing. It is worth noting that the temperature remained stable throughout the afternoon. The shadows shifted as the hours passed, a slow and predictable dance of light and dark. Ultimately, the day was a collection of such moments and observations, each one valid on its own, yet contributing to no overarching narrative or conclusion. This text serves only to fill the space designated for it.

\begin{figure}[H]     
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
  \label{fig:teaser}
\end{figure}



==> sections/method.tex <==
\section{Methodology}
\subsection{Secondary Level Headings}
\subsubsection{Three Level Headings}
\vspace{0.3pt}\noindent\textbf{Fourth Level Headings}\hspace{1ex}
This is used to test the format of the content.

==> sections/relatedwork.tex <==
\section{Related Work}
\subsection{Secondary Level Headings}
\subsubsection{Three Level Headings}
\vspace{0.3pt}\noindent\textbf{Fourth Level Headings}\hspace{1ex}
This is used to test the format of the content.

==> sections/results.tex <==
\section{Experiments and Results}
\subsection{Secondary Level Headings}
\subsubsection{Three Level Headings}
\vspace{0.3pt}\noindent\textbf{Fourth Level Headings}\hspace{1ex}
This is used to test the format of the content.

\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}
